Developing Assistive Technology to Support Reminiscence Therapy: A User-Centered Study to Identify Caregivers' Needs

Reminiscence therapy is an inexpensive non-pharmacological therapy commonly used due to its therapeutic value for PwD, as it can be used to promote independence, positive moods and behavior, and improve their quality of life. Caregivers are one of the main pillars in the adoption of digital technologies for reminiscence therapy, as they are responsible for its administration. Despite their comprehensive understanding of the needs and difficulties associated with the therapy, their perspective has not been fully taken into account in the development of existing technological solutions. To inform the design of technological solutions within dementia care, we followed a user-centered design approach through worldwide surveys, follow-up semi-structured interviews, and focus groups. Seven hundred and seven informal and 52 formal caregivers participated in our study. Our findings show that technological solutions must provide mechanisms to carry out the therapy in a simple way, reducing the amount of work for caregivers when preparing and conducting therapy sessions. They should also diversify and personalize the current session (and following ones) based on both the biographical information of the PwD and their emotional reactions. This is particularly important since the PwD often become agitated, aggressive or angry, and caregivers might not know how to properly deal with this situation (in particular, the informal ones). Additionally, formal caregivers need an easy way to manage information of the different PwD they take care of, and consult the history of sessions performed (in particular, to identify images that triggered negative emotional reactions, and consult any notes taken about them). As a result, we present a list of validated functional requirements gathered for the PwD and both formal and informal caregivers, as well as the corresponding expected primary and secondary outcomes.

==> lsb_2c.tex <==
        \begin{table}[!h]
	        \small	        
	        \renewcommand{\arraystretch}{1.2}
	        \captionsetup{labelformat=empty} 
    	    \begin{tabular}{p{74mm}}
    	        \textbf{Why caregivers do not create \ac{LSB}:}\\
    	        \toprule
    	        \textit{``Caregivers need more support. These ideas are helpful to the person with dementia, and indirectly to caregivers who find joy when their loved one is happy. Yet, way too much focus is on helping the person with dementia. As a caregiver I am very lonely and exhausted.''} [id-78]\\
    	        \textit{``Some easy way to sort, keep, file items would be appreciated. Since I am the caregiver 24 hours, take care of the house and the yard, and have to find time for myself to stay healthy, the Memory Book is a hit and miss.''} [id-95]\\
    	        \textit{``Many pictures react with her differently but it is hard to have time to organise memory books or to keep her interest in it. I tried to get family involved but they actually got bored of it quicker than mum!!! So, in the end, she gave up too. I want to carry on and do it for her to see later but I just don't have the time working and then going home.''} [id-264]\\
    	        \textit{``We are so busy just being able to get food made and to medical appointments that takes up all the energy for the day. So far, no time for hobbies, just TV with no effort involved.''} [id-353]
			    %``It is very difficult to have time to make memoirs when you are alone caring for a person with dementia and working full time. I think it's a good idea, but difficult to implement. For me the most important thing to relive memories at this time is to have her in an institution that truly has the time and availability to take care of her and stimulate what is very difficult and then I would have useful time to be with her there and make these memory books.'' [id-526] %, but this country makes these situations very difficult.
        	\end{tabular}
            \end{table}
